Topological properties of the [110] SnTe nanowires

SnTe materials are know to be a platform for realization of various strong and symmetry protected topological phases in one, two and three spatial dimensions. We study symmetry-protected topological states in $[110]$ SnTe nanowires in the presence of various combinations of Zeeman field, $s-$wave superconductivity, inversion-symmetry-breaking field and the thickness of the wire. In the normal state we find a Weyl semimetal phase protected by a twofold screw axis symmetry and a topological insulating phase characterized by a $\mathbb{Z}$ invariant protected by a mirror symmetry. In the presence of superconductivity, we find inversion-symmetry-protected gapless phase which becomes fully gapped and topologically non-trivial by introducing an inversion-symmetry-breaking field. Consequently, we find topologically protected localized Majorana zero modes appear at the ends of the wire. We find that this Majorana phase is much easier to achieve in a $[110]$ SnTe nanowire than in a $[001]$ one.

==> cover.tex <==
Dear Editor,

Please find enclosed our manuscript “Topological properties of the [101] SnTe nanowires”, which we submit to Physical Review B.
In our manuscript we study symmetry-protected topological states in [101] SnTe nanowires in the presence of various combinations of Zeeman field, s-wave superconductivity and inversion-symmetry-breaking field. 

SnTe materials are one of the most flexible material platforms for exploring the interplay of topology and different types of symmetry breaking. They are paradigmatic systems for studying 3D topological crystalline insulators and topological phase transitions, because the band inversion can be controlled with the Sn content. It is also predicted that the SnTe multilayer systems can support lower-dimensional topological phases, like quantum spin Hall and 2D topological crystalline insulator phases. Furthermore, SnTe materials are promising candidate systems for studying the higher order topology. 
	
On the other hand, SnTe materials are also one of the most flexible platforms for studying the interplay of various types of symmetry breaking fields. The superconductivity can be induced via the proximity effect or by In-doping. Interesting topological phases are predicted to arise also due to the time-reversal symmetry breaking. For instance Zeeman magnetic field can be efficiently applied  externally by taking advantage of the huge g factor g ≈ 50  or it can be introduced with the help of magnetic dopants. SnTe materials also  offer unique opportunities for breaking crystalline symmetries. In particular, it is possible to break the inversion symmetry by utilizing ferroelectricity or a structure inversion asymmetry. This has already enabled the realization of a giant Rashba effect, and it may be important also for the topology. 

So far the topological properties of SnTe nanowires have received little attention experimentally, but this may soon change due to the continuous progress in their fabrication. Therefore we believe that our manuscript will be a valuable contribution to this research field and it is well suited for the Physical Review B journal.


Thank you in advance for your kind consideration.

Sincerely Yours,
Alicja Kawala and Wojciech Brzezicki





==> referees.tex <==
Ewelina Hankiewicz, University of Wuerzburg, Germany, email: Hankiewicz@physik.uni-wuerzburg.de
Luis E. F. Foa Torres, Universidad  de  Chile, Santiago,  email: lfoa@ing.uchile.cl
Ion Cosma Fulga, IFW-Dresden, Germany, email: i.c.fulga@ifw-dresden.de
Paola Gentile, CNR-SPIN, Italy, email: paola.gentile@spin.cnr.it
Tom O'Brian, Leiden University, Netherlands,  email: obrien@lorentz.leidenuniv.nl
Bernard van Heck, Microsoft Quantum Lab Delft, Netherlands, bernard.vanheck@microsoft.com
Annica Black-Schaffer, Uppsala University, email: annica.black-schaffer@physics.uu.se

